SparseOcc: Rethinking Sparse Latent Representation for Vision-Based Semantic Occupancy Prediction

Vision-based perception for autonomous driving requires an explicit modeling of a 3D space, where 2D latent representations are mapped and subsequent 3D operators are applied. However, operating on dense latent spaces introduces a cubic time and space complexity, which limits scalability in terms of perception range or spatial resolution. Existing approaches compress the dense representation using projections like Bird's Eye View (BEV) or Tri-Perspective View (TPV). Although efficient, these projections result in information loss, especially for tasks like semantic occupancy prediction. To address this, we propose SparseOcc, an efficient occupancy network inspired by sparse point cloud processing. It utilizes a lossless sparse latent representation with three key innovations. Firstly, a 3D sparse diffuser performs latent completion using spatially decomposed 3D sparse convolutional kernels. Secondly, a feature pyramid and sparse interpolation enhance scales with information from others. Finally, the transformer head is redesigned as a sparse variant. SparseOcc achieves a remarkable 74.9% reduction on FLOPs over the dense baseline. Interestingly, it also improves accuracy, from 12.8% to 14.1% mIOU, which in part can be attributed to the sparse representation's ability to avoid hallucinations on empty voxels.

==> figure_tex/infer_memory.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=.55]{figures/infer_memory.pdf}
    \caption{\textbf{Efficiency analysis when scaling up the 3D representation on SemanticKITTI~\cite{semantickitti} validation set.} The left axis represents the inference GPU memory. The right axis denotes the number of voxels. The 3D downsampling ratio is considered between the ground-truth and the LSS output. The number of non-empty voxels is measured using max-donwsampled ground-truth.}
    \label{fig:infer_memory}
    \vspace{-10pt}
\end{figure}

==> figure_tex/sparseconv.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=.55]{figures/sparseconv.pdf}
    \vspace{-5pt}
    \caption{\textbf{Comparison between sparse submanifold convolution and sparse convolution.} For simplicity, 2D feature map and 2D kernels are utilized.}
    \label{fig:sparseconv}
    \vspace{-7pt}
\end{figure}

==> figure_tex/vis_kitti.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=.54]{figures/vis_kitti.pdf}
    \caption{\textbf{Qualitative results of 3D semantic scene completion on SemanticKITTI~\cite{semantickitti} validation set.}
    The input monocular image is shown on the left, and the 3D semantic scene completion results from OccFormer~\cite{occformer}, our SparseOcc, and the ground-truth are then visualized sequentially.}
    \label{fig:res_vis_kitti}
    \vspace{-10pt}
\end{figure*}

==> tables/abl_latency.tex <==
\begin{table}[!htbp]
  \centering
%   \setlength{\tabcolsep}{1.1mm} 
  \resizebox{0.46\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
          Dataset & Method &  IoU & mIoU  & Latency(s) & 3D Latency(s)\\
        \hline\hline
       \noalign{\smallskip}
       % - & 0 & - & 35.5 & 12.1 \\
       % \hline
       \multirow{3}{*}{[\textcolor{cyan}{32}]}
           & OpenOccupancy [\textcolor{cyan}{32}] & 19.3 & 10.3 & 1.22 & 0.84 \\
           % \cline{2-5}
           & C-CONet [\textcolor{cyan}{32}] & 20.1 &  12.8 & 2.58 & 2.18 \\
           % \cline{2-5}
           & SparseOcc [ours] & \textbf{21.8} & \textbf{14.4} & \textbf{0.25} & 0.19\\
        \hline
        \multirow{2}{*}{[\textcolor{cyan}{1}]}
           &  OccFormer [\textcolor{cyan}{39}]  & \textbf{36.5} & \textbf{13.5} & 0.31 & 0.24\\ 
           % \cline{2-5}
           &  SparseOcc [ours]  & \textbf{36.5} & 13.1 & \textbf{0.23} & 0.16\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \end{tabular}}
    \vspace{-3mm}
  \caption{Performance and latency comparison.} 
    \label{tab:abl_latency} % end caption
    \vspace{-5mm}
\end{table}

==> tables/nusc_lidarseg_val.tex <==
% \definecolor{nbarrier}{RGB}{255, 120, 50}
% \definecolor{nbicycle}{RGB}{255, 192, 203}
% \definecolor{nbus}{RGB}{255, 255, 0}
% \definecolor{ncar}{RGB}{0, 150, 245}
% \definecolor{nconstruct}{RGB}{0, 255, 255}
% \definecolor{nmotor}{RGB}{200, 180, 0}
% \definecolor{npedestrian}{RGB}{255, 0, 0}
% \definecolor{ntraffic}{RGB}{255, 240, 150}
% \definecolor{ntrailer}{RGB}{135, 60, 0}
% \definecolor{ntruck}{RGB}{160, 32, 240}
% \definecolor{ndriveable}{RGB}{255, 0, 255}
% \definecolor{nother}{RGB}{139, 137, 137}
% \definecolor{nsidewalk}{RGB}{75, 0, 75}
% \definecolor{nterrain}{RGB}{150, 240, 80}
% \definecolor{nmanmade}{RGB}{213, 213, 213}
% \definecolor{nvegetation}{RGB}{0, 175, 0}

\begin{table*}[ht]
    \footnotesize
    \setlength{\tabcolsep}{0.0045\linewidth}
    \newcommand{\classfreq}[1]{{~\tiny(\nuscenesfreq{#1}\%)}}  %
    \centering
    \begin{tabular}{l|c|c|c|c| c c c c c c c c c c c c c c c c}
    \toprule
    Method
    & \makecell{Input \\ Modality} & Backbone & \makecell{Image \\ Size} & mIoU
    & \rotatebox{90}{barrier}
    
    & \rotatebox{90}{bicycle}
    
    & \rotatebox{90}{bus}
    
    & \rotatebox{90}{car}
    
    & \rotatebox{90}{const. veh.}
    
    & \rotatebox{90}{motorcycle}
    
    & \rotatebox{90}{pedestrian}
    
    & \rotatebox{90}{traffic cone}
    
    & \rotatebox{90}{trailer}
    
    & \rotatebox{90}{truck}
    
    & \rotatebox{90}{drive. suf.}
    
    & \rotatebox{90}{other flat}
    
    & \rotatebox{90}{sidewalk}
    
    & \rotatebox{90}{terrain}
    
    & \rotatebox{90}{manmade}
    
    & \rotatebox{90}{vegetation}
    
    \\
    \midrule
    
    RangeNet++~\cite{rangenet++} & LiDAR & \multirow{4}{*}{-} & \multirow{4}{*}{-} &  65.5 & 66.0 & 21.3 & 77.2 & 80.9 & 30.2 & 66.8 & 69.6 &  52.1 & 54.2 & {72.3} & {94.1} & 66.6 & 63.5 & 70.1 & 83.1 & 79.8 \\
    
    PolarNet~\cite{zhang2020polarnet} & LiDAR &  &  & 71.0 & 74.7 & 28.2 & 85.3 & 90.9 & 35.1 & 77.5 & 71.3 & 58.8 & 57.4 & 76.1 & 96.5 & 71.1 & 74.7 & 74.0 & 87.3 & 85.7  \\
    
    Salsanext~\cite{Salsanext} & LiDAR & & & 72.2 & 74.8 & 34.1 & 85.9 & 88.4 & 42.2 & 72.4 & 72.2 & 63.1 & 61.3 & 76.5 & 96.0 & 70.8 & 71.2 & 71.5 & 86.7 & 84.4 \\
    
    {Cylinder3D}~\cite{cylindrical++} & LiDAR & & & \bf{76.1} & \bf{76.4} & \bf{40.3} & \bf{91.2} & \bf{93.8} & \textbf{51.3} & \bf{78.0} & \bf{78.9} & \bf{64.9} & \bf{62.1} & \bf{84.4} & \bf{96.8} & \bf{71.6} & \bf{76.4} & \bf{75.4} & \bf{90.5} & \bf{87.4}  \\
    \midrule	
    
    TPVFormer~\cite{tpvformer} & Camera & \multirow{3}{*}{R50} & 850$\times$450 & 59.3  & 64.9 & 27.0 & 83.0 & 82.8 & 38.3 & 27.4 & 44.9 & 24.0 & 55.4 & 73.6 & 91.7 & 60.7 & 59.8 & 61.1 & 78.2 & 76.5  \\ %

    OccFormer~\cite{occformer} & Camera & & 704$\times$256 & 68.1 & \textcolor{green}{69.2} & 36.9 & \textbf{91.2} & 84.4 & 47.3 & 59.1 & 61.9 & \textcolor{green}{42.1} & \textcolor{green}{58.8} & \textcolor{green}{82.8} & \textcolor{green}{93.0} & \textcolor{green}{67.5} & \textcolor{green}{67.4} & \textcolor{green}{68.5} & \textcolor{green}{81.0} & 78.5 \\

    {SparseOcc} (ours) & Camera & & 704$\times$256 & \textcolor{green}{68.4} & 69.1 & \textcolor{green}{40.4} & \textcolor{green}{89.1} & \textcolor{green}{85.0} & \textcolor{green}{49.9} & \textcolor{green}{71.0} & \textcolor{green}{62.0} & 38.1 & 58.1 & 79.4 & 92.9 & 65.8 & 66.2 & 67.0 & 80.9 & \textcolor{green}{78.9} \\
    
    % \midrule
    
    % BEVFormer~\cite{BEVFormer} & Camera & \multirow{3}{*}{\makecell{R101}} & \multirow{3}{*}{1600$\times$900} & 56.2 & 54.0 & 22.8 & 76.7 & 74.0 & 45.8 & 53.1 & 44.5 & 24.7 & 54.7 & 65.5 & 88.5 & 58.1 & 50.5 & 52.8 & 71.0 & 63.0  \\
    
    % TPVFormer~\cite{tpvformer} & Camera & & & 68.9  & 70.0 & 40.9 & 93.7 & 85.6 & 49.8 & 68.4 & 59.7 & 38.2 & 65.3 & 83.0 & 93.3 & 64.4 & 64.3 & 64.5 & 81.6 & 79.3  \\ %

    % \textbf{OccFormer} (ours) & Camera & & & 70.4 & 70.3 & 43.8 & 93.2 & 85.2 & 52.0 & 59.1 & 67.6 & 45.4 & 64.4 & 84.5 & 93.8 & 68.2 & 67.8 & 68.3 & 82.1 & 80.4\\
    
    \bottomrule
    \end{tabular}
    \caption{\textbf{LiDAR segmentation results on nuScenes validation set.} For vision-based methods, we list the utilized image backbone and the input image sizes. The \textbf{bold} numbers indicate the best results in the whole table and the \textcolor{green}{green} numbers indicate the best results in vision-based methods.}
    \label{tab:nusc_lidarseg_val}
\end{table*}

==> tables/rebuttal_adapation.tex <==
% \vspace{-3mm}
\begin{table}[!htbp]
  \centering
%   \setlength{\tabcolsep}{1.1mm} 
  \resizebox{0.27\textwidth}{!}{
    \begin{tabular}{c|c|c|c}
        \hline
        Method & Input & IoU & mIoU \\
        \hline\hline
        LMSCNet~[\textcolor{cyan}{27}] & C & 28.61 & 6.70 \\ %
        3DSketch~[\textcolor{cyan}{5}] & C & 33.30 & 7.50  \\ %
        AICNet~[\textcolor{cyan}{16}] & C & 29.59 & 8.31  \\ %
        %JS3C-Net~ & C & \textbf{38.98} & 10.31 \\
        \midrule
        SparseOcc & C & \textbf{36.48} & \textbf{13.12}  \\
        \hline
    \end{tabular}}\\
    \vspace{-3mm}
    \caption{LiDAR-based adaptations v.s. SparseOcc. }
    \label{table:re_adpt}
    \vspace{-4mm}
\end{table}
